AdaCoder: Adaptive Prompt Compression for Programmatic Visual Question Answering

Visual question answering aims to provide responses to natural language questions given visual input. Recently, visual programmatic models (VPMs), which generate executable programs to answer questions through large language models (LLMs), have attracted research interest. However, they often require long input prompts to provide the LLM with sufficient API usage details to generate relevant code. To address this limitation, we propose AdaCoder, an adaptive prompt compression framework for VPMs. AdaCoder operates in two phases: a compression phase and an inference phase. In the compression phase, given a preprompt that describes all API definitions in the Python language with example snippets of code, a set of compressed preprompts is generated, each depending on a specific question type. In the inference phase, given an input question, AdaCoder predicts the question type and chooses the appropriate corresponding compressed preprompt to generate code to answer the question. Notably, AdaCoder employs a single frozen LLM and pre-defined prompts, negating the necessity of additional training and maintaining adaptability across different powerful black-box LLMs such as GPT and Claude. In experiments, we apply AdaCoder to ViperGPT and demonstrate that it reduces token length by 71.1%, while maintaining or even improving the performance of visual question answering.

==> prompts/prompt_c.tex <==
        Examples
        --------
        >>> # return the foo
        >>> def execute_command(image) -> List[ImagePatch]:
        >>>     image_patch = ImagePatch(image)
        >>>     foo_patches = image_patch.find("foo")
        >>>     return foo_patches
        Examples
        -------
        >>> # Are there both foos and garply bars in the photo?
        >>> def execute_command(image)->str:
        >>>     image_patch = ImagePatch(image)
        >>>     is_foo = image_patch.exists("foo")
        >>>     is_garply_bar = image_patch.exists("garply bar")
        >>>     return bool_to_yesno(is_foo and is_garply_bar)

        Examples
        -------
        >>> # Do the letters have blue color?
        >>> def execute_command(image) -> str:
        >>>     image_patch = ImagePatch(image)
        >>>     letters_patches = image_patch.find("letters")
        >>>     # Question assumes only one letter patch
        >>>     return bool_to_yesno(letters_patches[0].verify_property("letters", "blue"))
        """

                Examples
        -------
        >>> # Is the foo gold or white?
        >>> def execute_command(image)->str:
        >>>     image_patch = ImagePatch(image)
        >>>     foo_patches = image_patch.find("foo")
        >>>     # Question assumes one foo patch
        >>>     return foo_patches[0].best_text_match(["gold", "white"])
        """

                Examples
        -------

        >>> # Which kind of baz is not fredding?
        >>> def execute_command(image) -> str:
        >>>     image_patch = ImagePatch(image)
        >>>     baz_patches = image_patch.find("baz")
        >>>     for baz_patch in baz_patches:
        >>>         if not baz_patch.verify_property("baz", "fredding"):
        >>>             return baz_patch.simple_query("What is this baz?")

        >>> # What color is the foo?
        >>> def execute_command(image) -> str:
        >>>     image_patch = ImagePatch(image)
        >>>     foo_patches = image_patch.find("foo")
        >>>     foo_patch = foo_patches[0]
        >>>     return foo_patch.simple_query("What is the color?")

        >>> # Is the second bar from the left quuxy?
        >>> def execute_command(image) -> str:
        >>>     image_patch = ImagePatch(image)
        >>>     bar_patches = image_patch.find("bar")
        >>>     bar_patches.sort(key=lambda x: x.horizontal_center)
        >>>     bar_patch = bar_patches[1]
        >>>     return bar_patch.simple_query("Is the bar quuxy?")

        Examples
        --------
        >>> # the bar furthest away
        >>> def execute_command(image)->ImagePatch:
        >>>     image_patch = ImagePatch(image)
        >>>     bar_patches = image_patch.find("bar")
        >>>     bar_patches.sort(key=lambda bar: bar.compute_depth())
        >>>     return bar_patches[-1]

        Examples
        -------
        >>> # What is in upper left of the image?
        >>> def execute_command(image)->ImagePatch:
        >>>     image_patch = ImagePatch(image)
        >>>     upper_left_patch = image_patch.crop(image_patch.left, round((image_patch.upper+image_patch.lower)/2), round((image_patch.left+image_patch.right)/2), image_patch.upper)
        >>>     return upper_left_patch.simple_query("What is it?")


        Examples
        --------
        >>> # black foo on top of the qux
        >>> def execute_command(image) -> ImagePatch:
        >>>     image_patch = ImagePatch(image)
        >>>     qux_patches = image_patch.find("qux")
        >>>     qux_patch = qux_patches[0]
        >>>     foo_patches = image_patch.find("black foo")
        >>>     for foo_patch in foo_patches:
        >>>         if foo_patch.vertical_center > qux_patch.vertical_center and foo_patch.overlaps_with(qux_patch.left, qux_patch.lower, qux_patch.right, qux_patch.upper):
        >>>             return foo

        Examples
        --------
        >>> # What is the city this building is in?
        >>> def execute_command(image) -> str:
        >>>     image_patch = ImagePatch(image)
        >>>     building_patches = image_patch.find("building")
        >>>     building_patch = building_patches[0]
        >>>     building_name = building_patch.simple_query("What is the name of the building?")
        >>>     return building_patch.llm_query(f"What city is {building_name} in?", long_answer=False)

        >>> # Who invented this object?
        >>> def execute_command(image) -> str:
        >>>     image_patch = ImagePatch(image)
        >>>     object_patches = image_patch.find("object")
        >>>     object_patch = object_patches[0]
        >>>     object_name = object_patch.simple_query("What is the name of the object?")
        >>>     return object_patch.llm_query(f"Who invented {object_name}?", long_answer=False)

        >>> # Explain the history behind this object.
        >>> def execute_command(image) -> str:
        >>>     image_patch = ImagePatch(image)
        >>>     object_patches = image_patch.find("object")
        >>>     object_patch = object_patches[0]
        >>>     object_name = object_patch.simple_query("What is the name of the object?")
        >>>     return object_patch.llm_query(f"What is the history behind {object_name}?", long_answer=True)


        Examples
    --------
    >>> # What is the blue foo doing?
    >>> def execute_command(image) -> str:
    >>>     image_patch = ImagePatch(image)
    >>>     foo_patches = image_patch.find("foo")
    >>>     foo_patch = best_image_match(foo_patches, ["blue"])
    >>>     return foo_patch.simple_query("What is the foo doing?")

    Examples
    --------
    >>> # Return the qux that is closest to the foo
    >>> def execute_command(image):
    >>>     image_patch = ImagePatch(image)
    >>>     qux_patches = image_patch.find('qux')
    >>>     foo_patches = image_patch.find('foo')
    >>>     foo_patch = foo_patches[0]
    >>>     qux_patches.sort(key=lambda x: distance(x, foo_patch))
    >>>     return qux_patches[0]

    Examples
    --------
    >>> # Is the buz green?
    >>> def execute_command(image):
    >>>     image_patch = ImagePatch(image)
    >>>     buz_patches = image_patch.find('buz')
    >>>     buz_patch = best_image_match(buz_patches, ["buz"])
    >>>     return bool_to_yesno(buz_patch.verify_property("buz", "green"))

==> prompts/prompt_pcls.tex <==
\begin{minted}[breaklines, breaksymbolleft={}, breaksymbolright={}, fontsize=\footnotesize, escapeinside=||]{markdown}
Classify the question into following question classes.

- {type[0]}: {type_definition[0]}
- {type[1]}: {type_definition[1]}
...
- {type[n]}: {type_definition[n]}

Question: 
\end{minted}

==> prompts/prompt_pdef.tex <==
\begin{minted}[bgcolor=black!5!white, breaklines, breaksymbolleft={}, breaksymbolright={}, fontsize=\scriptsize, escapeinside=||]{markdown}
import math

class ImagePatch:
    """A Python class containing a crop of an image centered around a particular object, as well as relevant information.
    Attributes
    ----------
    cropped_image : array_like
        An array-like of the cropped image taken from the original image.
    left, lower, right, upper : int
        An int describing the position of the (left/lower/right/upper) border of the crop's bounding box in the original image.

    Methods
    -------
    find(object_name: str)->List[ImagePatch]
        Returns a list of new ImagePatch objects containing crops of the image centered around any objects found in the
        image matching the object_name.
    exists(object_name: str)->bool
        Returns True if the object specified by object_name is found in the image, and False otherwise.
    verify_property(property: str)->bool
        Returns True if the property is met, and False otherwise.
    best_text_match(option_list: List[str], prefix: str)->str
        Returns the string that best matches the image.
    simple_query(question: str=None)->str
        Returns the answer to a basic question asked about the image. If no question is provided, returns the answer to "What is this?".
    llm_query(question: str, long_answer: bool)->str
        References a large language model (e.g., GPT) to produce a response to the given question. Default is short-form answers, can be made long-form responses with the long_answer flag.
    compute_depth()->float
        Returns the median depth of the image crop.
    crop(left: int, lower: int, right: int, upper: int)->ImagePatch
        Returns a new ImagePatch object containing a crop of the image at the given coordinates.
    """

    def __init__(self, image, left: int = None, lower: int = None, right: int = None, upper: int = None):
        """Initializes an ImagePatch object by cropping the image at the given coordinates and stores the coordinates as
        attributes. If no coordinates are provided, the image is left unmodified, and the coordinates are set to the
        dimensions of the image.
        Parameters
        -------
        image : array_like
            An array-like of the original image.
        left, lower, right, upper : int
            An int describing the position of the (left/lower/right/upper) border of the crop's bounding box in the original image.
        """
        if left is None and right is None and upper is None and lower is None:
            self.cropped_image = image
            self.left = 0
            self.lower = 0
            self.right = image.shape[2]  # width
            self.upper = image.shape[1]  # height
        else:
            self.cropped_image = image[:, lower:upper, left:right]
            self.left = left
            self.upper = upper
            self.right = right
            self.lower = lower

        self.width = self.cropped_image.shape[2]
        self.height = self.cropped_image.shape[1]

        self.horizontal_center = (self.left + self.right) / 2
        self.vertical_center = (self.lower + self.upper) / 2

    def find(self, object_name: str) -> List[ImagePatch]:
        """Returns a list of ImagePatch objects matching object_name contained in the crop if any are found.
        Otherwise, returns an empty list.
        Parameters
        ----------
        object_name : str
            the name of the object to be found

        Returns
        -------
        List[ImagePatch]
            a list of ImagePatch objects matching object_name contained in the crop

        """
        return find_in_image(self.cropped_image, object_name)

    def exists(self, object_name: str) -> bool:
        """Returns True if the object specified by object_name is found in the image, and False otherwise.
        Parameters
        -------
        object_name : str
            A string describing the name of the object to be found in the image.

        """
        return len(self.find(object_name)) > 0

    def verify_property(self, object_name: str, visual_property: str) -> bool:
        """Returns True if the object possesses the visual property, and False otherwise.
        Differs from 'exists' in that it presupposes the existence of the object specified by object_name, instead checking whether the object possesses the property.
        Parameters
        -------
        object_name : str
            A string describing the name of the object to be found in the image.
        visual_property : str
            A string describing the simple visual property (e.g., color, shape, material) to be checked.

        """

        return verify_property(self.cropped_image, object_name, property)

    def best_text_match(self, option_list: List[str]) -> str:
        """Returns the string that best matches the image.
        Parameters
        -------
        option_list : str
            A list with the names of the different options
        prefix : str
            A string with the prefixes to append to the options

        """

        return best_text_match(self.cropped_image, option_list)

    def simple_query(self, question: str = None) -> str:
        """Returns the answer to a basic question asked about the image. If no question is provided, returns the answer
        to "What is this?". The questions are about basic perception, and are not meant to be used for complex reasoning
        or external knowledge.
        Parameters
        -------
        question : str
            A string describing the question to be asked.

        """
        return simple_query(self.cropped_image, question)

    def compute_depth(self):
        """Returns the median depth of the image crop
        Parameters
        ----------
        Returns
        -------
        float
            the median depth of the image crop

        """
        depth_map = compute_depth(self.cropped_image)
        return depth_map.median()

    def crop(self, left: int, lower: int, right: int, upper: int) -> ImagePatch:
        """Returns a new ImagePatch cropped from the current ImagePatch.
        Parameters
        -------
        left, lower, right, upper : int
            The (left/lower/right/upper)most pixel of the cropped image.
            
        Returns
        -------
        ImagePatch
            New ImagePatch cropped from the current ImagePatch.
            
        """
        return ImagePatch(self.cropped_image, left, lower, right, upper)

    def overlaps_with(self, left, lower, right, upper) -> bool:
        """Returns True if a crop with the given coordinates overlaps with this one,
        else False.
        Parameters
        ----------
        left, lower, right, upper : int
            the (left/lower/right/upper) border of the crop to be checked

        Returns
        -------
        bool
            True if a crop with the given coordinates overlaps with this one, else False

        """
        return self.left <= right and self.right >= left and self.lower <= upper and self.upper >= lower

    def llm_query(self, question: str, long_answer: bool = True) -> str:
        """Answers a text question using GPT-3. The input question is always a formatted string with a variable in it.

        Parameters
        ----------
        question: str
            the text question to ask. Must not contain any reference to 'the image' or 'the photo', etc.
        long_answer: bool
            whether to return a short answer or a long answer. Short answers are one or at most two words, very concise.
            Long answers are longer, and may be paragraphs and explanations. Defalt is True (so long answer).

        """
        return llm_query(question, long_answer)


def best_image_match(list_patches: List[ImagePatch], content: List[str], return_index=False) -> Union[ImagePatch, int]:
    """Returns the patch most likely to contain the content.
    Parameters
    ----------
    list_patches : List[ImagePatch]
    content : List[str]
        the object of interest
    return_index : bool
        if True, returns the index of the patch most likely to contain the object

    Returns
    -------
    int
        Patch most likely to contain the object
        
    """
    return best_image_match(list_patches, content, return_index)


def distance(patch_a: ImagePatch, patch_b: ImagePatch) -> float:
    """
    Returns the distance between the edges of two ImagePatches. If the patches overlap, it returns a negative distance
    corresponding to the negative intersection over union.

    Parameters
    ----------
    patch_a : ImagePatch
    patch_b : ImagePatch
    
    Returns
    ----------
    float
        The distance of the two patches.

    """
    return distance(patch_a, patch_b)


def bool_to_yesno(bool_answer: bool) -> str:
    """
    Convert a boolean value to "yes" or "no"

    Parameters
    ----------
    bool_answer : bool
    
    Returns
    ----------
    str
        "yes" or "no"

    """
    return "yes" if bool_answer else "no"


def coerce_to_numeric(string):
    """
    This function takes a string as input and returns a float after removing any non-numeric characters.
    If the input string contains a range (e.g. "10-15"), it returns the first value in the range.
    """
    return coerce_to_numeric(string)

Write a function using Python and the ImagePatch class (above) that could be executed to provide an answer to the query. 

Consider the following guidelines:
- Use base Python (comparison, sorting) for basic logical operations, left/right/up/down, math, etc.
- Use the llm_query function to access external information and answer informational questions not concerning the image.

Query: INSERT_QUERY_HERE
\end{minted}

==> prompts/prompt_pdef_short.tex <==
\begin{minted}[bgcolor=black!5!white, breaklines, breaksymbolleft={}, breaksymbolright={}, fontsize=\scriptsize, escapeinside=||]{markdown}
|\defs{import}| |\others{math}|

|\defs{class} \classname{ImagePatch}|:
    |\coms{"""A Python class containing a crop of an image centered around a particular object, as well as relevant information.}|
    |\coms{...}|

    |\defs{def} \methodname{\_\_init\_\_}\others{(}\defs{self}\others{,} \others{image}\others{,} \others{left}: \intname{int} \others{=} \nonename{None}\others{,} \others{lower}\others{:} \intname{int} \others{=} \nonename{None}\others{,}|
                 |\others{right}\others{:} \intname{int} \others{=} \nonename{None}\others{,} \others{upper}\others{:} \intname{int} \others{=} \nonename{None})\others{:}|
        |\coms{"""Initializes an ImagePatch object by cropping the image at the given coordinates and stores the coordinates as attributes. If no coordinates are provided, the image is left unmodified, and the coordinates are set to the dimensions of the image.}|
        |\coms{...}|

|\defs{def} \methodname{best\_image\_match}\others{(}\others{list\_patches}\others{:} \intname{List}\others{[}\intname{ImagePatch}\others{]}\others{,} \others{content}\others{:} \intname{List}\others{[}\intname{str}\others{]}\others{,}|
                     |\others{return\_index}\others{ = }\nonename{False}\others{)} \others{->} \intname{Union}\others{[}\intname{ImagePatch}\others{,} \intname{int}\others{]}\others{:}|
    |\coms{"""Returns the patch most likely to contain the content.}|
    |\coms{Parameters}|
    |\coms{----------}|
    |\coms{list\_patches : List[ImagePatch]}|
    |\coms{...}|                                       |\normalfont{\small{\textbf{1,971 tokens, 9,299 characters}}}|
\end{minted}

==> prompts/prompt_pdef_short_v0.tex <==
\begin{minted}[bgcolor=black!5!white, breaklines, breaksymbolleft={}, breaksymbolright={}, fontsize=\scriptsize, escapeinside=||]{markdown}
import math

|\others{class} \classname{ImagePatch}|:
    """A Python class containing a crop of an image centered around a particular object, as well as relevant information.
    Attributes
...
    def |\methodname{\_\_init\_\_}\others{(}\varname{self}, image, left: int = None, lower: int = None, right: int = None, upper: int = None)|:
        """Initializes an ImagePatch object by cropping the image at the given coordinates and stores the coordinates as
        attributes. If no coordinates are provided, the image is left unmodified, and the coordinates are set to the
        dimensions of the image.
        Parameters
        -------
        image : array_like
            An array-like of the original image.
...

def best_image_match(list_patches: List[ImagePatch], content: List[str], return_index=False) -> Union[ImagePatch, int]:
    """Returns the patch most likely to contain the content.
    Parameters
    ----------
    list_patches : List[ImagePatch]
    content : List[str]
        the object of interest
    return_index : bool
        if True, returns the index of the patch most likely to contain the object
...                                           |\normalfont{\small{\textbf{1,971 tokens, 9,299 characters}}}|
\end{minted}

==> prompts/prompt_pdefhat.tex <==
\begin{minted}[breaklines, breaksymbolleft={}, breaksymbolright={}, fontsize=\scriptsize, escapeinside=||]{markdown}
API Reference:

Class: ImagePatch

Attributes:
- cropped_image: array_like - An array-like of the cropped image taken from the original image.
- left: int - The position of the left border of the crop's bounding box in the original image.
- lower: int - The position of the lower border of the crop's bounding box in the original image.
- right: int - The position of the right border of the crop's bounding box in the original image.
- upper: int - The position of the upper border of the crop's bounding box in the original image.
- width: int - The width of the cropped image.
- height: int - The height of the cropped image.
- horizontal_center: float - The horizontal center of the cropped image.
- vertical_center: float - The vertical center of the cropped image.

Methods:
- find(object_name: str) -> List[ImagePatch]: Returns a list of ImagePatch objects matching object_name contained in the crop.
- exists(object_name: str) -> bool: Returns True if the object specified by object_name is found in the image, and False otherwise.
- verify_property(object_name: str, visual_property: str) -> bool: Returns True if the object possesses the visual property, and False otherwise.
- best_text_match(option_list: List[str]) -> str: Returns the string that best matches the image.
- simple_query(question: str = None) -> str: Returns the answer to a basic question asked about the image.
- compute_depth() -> float: Returns the median depth of the image crop.
- crop(left: int, lower: int, right: int, upper: int) -> ImagePatch: Returns a new ImagePatch cropped from the current ImagePatch.
- overlaps_with(left: int, lower: int, right: int, upper: int) -> bool: Returns True if a crop with the given coordinates overlaps with this one, else False.
- llm_query(question: str, long_answer: bool = True) -> str: Answers a text question using GPT-3.

Functions:
- best_image_match(list_patches: List[ImagePatch], content: List[str], return_index=False) -> Union[ImagePatch, int]: Returns the patch most likely to contain the content.
- distance(patch_a: ImagePatch, patch_b: ImagePatch) -> float: Returns the distance between the edges of two ImagePatches.
- bool_to_yesno(bool_answer: bool) -> str: Convert a boolean value to "yes" or "no".
- coerce_to_numeric(string) -> float: Returns a float after removing any non-numeric characters from the input string.
\end{minted}

==> prompts/prompt_pdefhat_.tex <==
\begin{minted}[bgcolor=black!5!white, breaklines, breaksymbolleft={}, breaksymbolright={}, fontsize=\scriptsize, escapeinside=||]{markdown}
|\methodname{open\_image}\others{(}\varname{path}\others{: }\classname{str}\others{) -> }\classname{Image}|
API Reference:

Class: ImagePatch

Attributes:
- |\methodname{cropped\_image}|: |\classname{array\_like}| - An array-like of the cropped image taken from the
  original image.
- left: |\classname{int}| - The position of the left border of the crop's bounding box in the
  original image.
- |\methodname{lower}|: |\classname{int}| - The position of the lower border of the crop's bounding box in
  the original image.
- |\methodname{right}|: |\classname{int}| - The position of the right border of the crop's bounding box in
  the original image.
- |\methodname{upper}|: |\classname{int}| - The position of the upper border of the crop's bounding box in
  the original image.
- |\methodname{width}|: |\classname{int}| - The width of the cropped image.
- |\methodname{height}|: |\classname{int}| - The height of the cropped image.
- |\methodname{horizontal\_center}|: |\classname{float}| - The horizontal center of the cropped image.
- |\methodname{vertical\_center}|: |\classname{float}| - The vertical center of the cropped image.

Methods:
- |\methodname{find}\others{(}\varname{object\_name}\others{:} \classname{str}\others{) -> }\classname{List}\others{[}\classname{ImagePatch}\others{]}|: Returns a list of ImagePatch
  objects matching object_name contained in the crop.
- |\methodname{exists}\others{(}\varname{object\_name}\others{:} \classname{str}\others{) -> }\classname{bool}|: Returns True if the object specified by
  object_name is found in the image, and False otherwise.
- |\methodname{verify\_property}\others{(}\varname{object\_name}\others{:} \classname{str}\others{, }\varname{visual\_property}\others{:} \classname{str}\others{) -> }\classname{bool}|: Returns
  True if the object possesses the visual property, and False otherwise.
- best_text_match(option_list: List[str]) -> str: Returns the string that best matches the image.
- simple_query(question: str = None) -> str: Returns the answer to a basic question asked about the image.
- compute_depth() -> float: Returns the median depth of the image crop.
- crop(left: int, lower: int, right: int, upper: int) -> ImagePatch: Returns a new ImagePatch cropped from the current ImagePatch.
- overlaps_with(left: int, lower: int, right: int, upper: int) -> bool: Returns True if a crop with the given coordinates overlaps with this one, else False.
- llm_query(question: str, long_answer: bool = True) -> str: Answers a text question using GPT-3.

Functions:
- |\methodname{best\_image\_match}\others{(}\varname{list\_patches}\others{:} \classname{List}\others{[}\classname{ImagePatch}\others{],} \varname{content}\others{:} \classname{List}\others{[}\classname{str}\others{],}|
  |\varname{return\_index}\others{=}\clasname{False}\others{) -> }\classname{Union}\others{[}\classname{ImagePatch}\others{,} \classname{int}\others{]}|: Returns the patch most likely to contain the content.
- |\methodname{distance}\others{(}\varname{patch\_a}\others{:} \classname{ImagePatch}\others{,} \varname{patch\_b}\others{:} \classname{ImagePatch}\others{) ->} \classname{float}|: Returns the
  distance between the edges of two ImagePatches.
- bool_to_yesno(bool_answer: bool) -> str: Convert a boolean value to "yes" or "no".
- coerce_to_numeric(string) -> float: Returns a float after removing any non-numeric characters from the input string.
\end{minted}

==> prompts/prompt_pdefhat_short.tex <==
\begin{minted}[bgcolor=black!5!white, breaklines, breaksymbolleft={}, breaksymbolright={}, fontsize=\scriptsize, escapeinside=||]{markdown}
|\varname{API Reference:}|

|\varname{Class:}| |\classname{ImagePatch}|

|\varname{Attributes:}|
|\ohters{-}| |\methodname{cropped\_image}\others{:} \intname{array\_like}| |\ohters{-}| |\coms{An array-like of the cropped image taken from the}|
  |\coms{original image.}|
|\ohters{-}| |\methodname{left}\others{:} \intname{int}| |\ohters{-}| |\coms{The position of the left border of the crop's bounding box in the}|
  |\coms{original image.}|
  ...

|\varname{Methods:}|
|\ohters{-}| |\methodname{find}\others{(}\others{object\_name}\others{:} \intname{str}\others{) -> }\intname{List}\others{[}\classname{ImagePatch}\others{]}|: |\coms{Returns a list of ImagePatch}|
  |\coms{objects matching object\_name contained in the crop.}|
|\ohters{-}| |\methodname{exists}\others{(}\others{object\_name}\others{:} \intname{str}\others{) -> }\intname{bool}|: |\coms{Returns True if the object specified by}|
  |\coms{object\_name is found in the image, and False otherwise.}|
  ...

|\varname{Functions:}|
|\ohters{-}| |\methodname{best\_image\_match}\others{(}\others{list\_patches}\others{:} \intname{List}\others{[}\intname{ImagePatch}\others{],} \others{content}\others{:} \intname{List}\others{[}\intname{str}\others{],}|
  |\others{return\_index}\others{=}\nonename{False}\others{) -> }\intname{Union}\others{[}\intname{ImagePatch}\others{,} \intname{int}\others{]}|: |\coms{Returns the patch most likely}| |\coms{to contain the content.}|
|\ohters{-}| |\methodname{distance}\others{(}\others{patch\_a}\others{:} \intname{ImagePatch}\others{,} \others{patch\_b}\others{:} \intname{ImagePatch}\others{) ->} \intname{float}|: |\coms{Returns the}|
  |\coms{distance between the edges of two ImagePatches.}|
  ...                                         |\normalfont{\small{\textbf{541 tokens, 2,360 characters}}}|
\end{minted}


==> prompts/prompt_pdefhat_short_v0.tex <==
\begin{minted}[bgcolor=black!5!white, breaklines, breaksymbolleft={}, breaksymbolright={}, fontsize=\scriptsize, escapeinside=||]{markdown}
API Reference:

Class: ImagePatch

Attributes:
- |\methodname{cropped\_image}|: |\classname{array\_like}| - An array-like of the cropped image taken from the
  original image.
- left: |\classname{int}| - The position of the left border of the crop's bounding box in the
  original image.
- |\methodname{lower}|: |\classname{int}| - The position of the lower border of the crop's bounding box in
  the original image.
...

Methods:
- |\methodname{find}\others{(}\varname{object\_name}\others{:} \classname{str}\others{) -> }\classname{List}\others{[}\classname{ImagePatch}\others{]}|: Returns a list of ImagePatch
  objects matching object_name contained in the crop.
- |\methodname{exists}\others{(}\varname{object\_name}\others{:} \classname{str}\others{) -> }\classname{bool}|: Returns True if the object specified by
  object_name is found in the image, and False otherwise.
- |\methodname{verify\_property}\others{(}\varname{object\_name}\others{:} \classname{str}\others{, }\varname{visual\_property}\others{:} \classname{str}\others{) -> }\classname{bool}|: Returns
  True if the object possesses the visual property, and False otherwise.
...

Functions:
- |\methodname{best\_image\_match}\others{(}\varname{list\_patches}\others{:} \classname{List}\others{[}\classname{ImagePatch}\others{],} \varname{content}\others{:} \classname{List}\others{[}\classname{str}\others{],}|
  |\varname{return\_index}\others{=}\clasname{False}\others{) -> }\classname{Union}\others{[}\classname{ImagePatch}\others{,} \classname{int}\others{]}|: Returns the patch most likely to contain the content.
- |\methodname{distance}\others{(}\varname{patch\_a}\others{:} \classname{ImagePatch}\others{,} \varname{patch\_b}\others{:} \classname{ImagePatch}\others{) ->} \classname{float}|: Returns the
  distance between the edges of two ImagePatches.
...                                           |\normalfont{\small{\textbf{541 tokens, 2,360 characters}}}|
\end{minted}


==> prompts/prompt_ppre.tex <==
\begin{minted}[bgcolor=black!5!white, breaklines, breaksymbolleft={}, breaksymbolright={}, fontsize=\scriptsize, escapeinside=||]{markdown}
import math

class ImagePatch:
    """A Python class containing a crop of an image centered around a particular object, as well as relevant information.
    Attributes
    ----------
    cropped_image : array_like
        An array-like of the cropped image taken from the original image.
    left, lower, right, upper : int
        An int describing the position of the (left/lower/right/upper) border of the crop's bounding box in the original image.

    Methods
    -------
    find(object_name: str)->List[ImagePatch]
        Returns a list of new ImagePatch objects containing crops of the image centered around any objects found in the
        image matching the object_name.
    exists(object_name: str)->bool
        Returns True if the object specified by object_name is found in the image, and False otherwise.
    verify_property(property: str)->bool
        Returns True if the property is met, and False otherwise.
    best_text_match(option_list: List[str], prefix: str)->str
        Returns the string that best matches the image.
    simple_query(question: str=None)->str
        Returns the answer to a basic question asked about the image. If no question is provided, returns the answer to "What is this?".
    llm_query(question: str, long_answer: bool)->str
        References a large language model (e.g., GPT) to produce a response to the given question. Default is short-form answers, can be made long-form responses with the long_answer flag.
    compute_depth()->float
        Returns the median depth of the image crop.
    crop(left: int, lower: int, right: int, upper: int)->ImagePatch
        Returns a new ImagePatch object containing a crop of the image at the given coordinates.
    """

    def __init__(self, image, left: int = None, lower: int = None, right: int = None, upper: int = None):
        """Initializes an ImagePatch object by cropping the image at the given coordinates and stores the coordinates as
        attributes. If no coordinates are provided, the image is left unmodified, and the coordinates are set to the
        dimensions of the image.
        Parameters
        -------
        image : array_like
            An array-like of the original image.
        left, lower, right, upper : int
            An int describing the position of the (left/lower/right/upper) border of the crop's bounding box in the original image.
        """
        if left is None and right is None and upper is None and lower is None:
            self.cropped_image = image
            self.left = 0
            self.lower = 0
            self.right = image.shape[2]  # width
            self.upper = image.shape[1]  # height
        else:
            self.cropped_image = image[:, lower:upper, left:right]
            self.left = left
            self.upper = upper
            self.right = right
            self.lower = lower

        self.width = self.cropped_image.shape[2]
        self.height = self.cropped_image.shape[1]

        self.horizontal_center = (self.left + self.right) / 2
        self.vertical_center = (self.lower + self.upper) / 2

    def find(self, object_name: str) -> List[ImagePatch]:
        """Returns a list of ImagePatch objects matching object_name contained in the crop if any are found.
        Otherwise, returns an empty list.
        Parameters
        ----------
        object_name : str
            the name of the object to be found

        Returns
        -------
        List[ImagePatch]
            a list of ImagePatch objects matching object_name contained in the crop

        Examples
        --------
        >>> # return the foo
        >>> def execute_command(image) -> List[ImagePatch]:
        >>>     image_patch = ImagePatch(image)
        >>>     foo_patches = image_patch.find("foo")
        >>>     return foo_patches
        """
        return find_in_image(self.cropped_image, object_name)

    def exists(self, object_name: str) -> bool:
        """Returns True if the object specified by object_name is found in the image, and False otherwise.
        Parameters
        -------
        object_name : str
            A string describing the name of the object to be found in the image.

        Examples
        -------
        >>> # Are there both foos and garply bars in the photo?
        >>> def execute_command(image)->str:
        >>>     image_patch = ImagePatch(image)
        >>>     is_foo = image_patch.exists("foo")
        >>>     is_garply_bar = image_patch.exists("garply bar")
        >>>     return bool_to_yesno(is_foo and is_garply_bar)
        """
        return len(self.find(object_name)) > 0

    def verify_property(self, object_name: str, visual_property: str) -> bool:
        """Returns True if the object possesses the visual property, and False otherwise.
        Differs from 'exists' in that it presupposes the existence of the object specified by object_name, instead checking whether the object possesses the property.
        Parameters
        -------
        object_name : str
            A string describing the name of the object to be found in the image.
        visual_property : str
            A string describing the simple visual property (e.g., color, shape, material) to be checked.

        Examples
        -------
        >>> # Do the letters have blue color?
        >>> def execute_command(image) -> str:
        >>>     image_patch = ImagePatch(image)
        >>>     letters_patches = image_patch.find("letters")
        >>>     # Question assumes only one letter patch
        >>>     return bool_to_yesno(letters_patches[0].verify_property("letters", "blue"))
        """
        return verify_property(self.cropped_image, object_name, property)

    def best_text_match(self, option_list: List[str]) -> str:
        """Returns the string that best matches the image.
        Parameters
        -------
        option_list : str
            A list with the names of the different options
        prefix : str
            A string with the prefixes to append to the options

        Examples
        -------
        >>> # Is the foo gold or white?
        >>> def execute_command(image)->str:
        >>>     image_patch = ImagePatch(image)
        >>>     foo_patches = image_patch.find("foo")
        >>>     # Question assumes one foo patch
        >>>     return foo_patches[0].best_text_match(["gold", "white"])
        """
        return best_text_match(self.cropped_image, option_list)

    def simple_query(self, question: str = None) -> str:
        """Returns the answer to a basic question asked about the image. If no question is provided, returns the answer
        to "What is this?". The questions are about basic perception, and are not meant to be used for complex reasoning
        or external knowledge.
        Parameters
        -------
        question : str
            A string describing the question to be asked.

        Examples
        -------

        >>> # Which kind of baz is not fredding?
        >>> def execute_command(image) -> str:
        >>>     image_patch = ImagePatch(image)
        >>>     baz_patches = image_patch.find("baz")
        >>>     for baz_patch in baz_patches:
        >>>         if not baz_patch.verify_property("baz", "fredding"):
        >>>             return baz_patch.simple_query("What is this baz?")

        >>> # What color is the foo?
        >>> def execute_command(image) -> str:
        >>>     image_patch = ImagePatch(image)
        >>>     foo_patches = image_patch.find("foo")
        >>>     foo_patch = foo_patches[0]
        >>>     return foo_patch.simple_query("What is the color?")

        >>> # Is the second bar from the left quuxy?
        >>> def execute_command(image) -> str:
        >>>     image_patch = ImagePatch(image)
        >>>     bar_patches = image_patch.find("bar")
        >>>     bar_patches.sort(key=lambda x: x.horizontal_center)
        >>>     bar_patch = bar_patches[1]
        >>>     return bar_patch.simple_query("Is the bar quuxy?")
        """
        return simple_query(self.cropped_image, question)

    def compute_depth(self):
        """Returns the median depth of the image crop
        Parameters
        ----------
        Returns
        -------
        float
            the median depth of the image crop

        Examples
        --------
        >>> # the bar furthest away
        >>> def execute_command(image)->ImagePatch:
        >>>     image_patch = ImagePatch(image)
        >>>     bar_patches = image_patch.find("bar")
        >>>     bar_patches.sort(key=lambda bar: bar.compute_depth())
        >>>     return bar_patches[-1]
        """
        depth_map = compute_depth(self.cropped_image)
        return depth_map.median()

    def crop(self, left: int, lower: int, right: int, upper: int) -> ImagePatch:
        """Returns a new ImagePatch cropped from the current ImagePatch.
        Parameters
        -------
        left, lower, right, upper : int
            The (left/lower/right/upper)most pixel of the cropped image.
            
        Returns
        -------
        ImagePatch
            New ImagePatch cropped from the current ImagePatch.
            
        Examples
        -------
        >>> # What is in upper left of the image?
        >>> def execute_command(image)->ImagePatch:
        >>>     image_patch = ImagePatch(image)
        >>>     upper_left_patch = image_patch.crop(image_patch.left, round((image_patch.upper+image_patch.lower)/2), round((image_patch.left+image_patch.right)/2), image_patch.upper)
        >>>     return upper_left_patch.simple_query("What is it?")
        """
        return ImagePatch(self.cropped_image, left, lower, right, upper)

    def overlaps_with(self, left, lower, right, upper) -> bool:
        """Returns True if a crop with the given coordinates overlaps with this one,
        else False.
        Parameters
        ----------
        left, lower, right, upper : int
            the (left/lower/right/upper) border of the crop to be checked

        Returns
        -------
        bool
            True if a crop with the given coordinates overlaps with this one, else False

        Examples
        --------
        >>> # black foo on top of the qux
        >>> def execute_command(image) -> ImagePatch:
        >>>     image_patch = ImagePatch(image)
        >>>     qux_patches = image_patch.find("qux")
        >>>     qux_patch = qux_patches[0]
        >>>     foo_patches = image_patch.find("black foo")
        >>>     for foo_patch in foo_patches:
        >>>         if foo_patch.vertical_center > qux_patch.vertical_center and foo_patch.overlaps_with(qux_patch.left, qux_patch.lower, qux_patch.right, qux_patch.upper):
        >>>             return foo
        """
        return self.left <= right and self.right >= left and self.lower <= upper and self.upper >= lower

    def llm_query(self, question: str, long_answer: bool = True) -> str:
        """Answers a text question using GPT-3. The input question is always a formatted string with a variable in it.

        Parameters
        ----------
        question: str
            the text question to ask. Must not contain any reference to 'the image' or 'the photo', etc.
        long_answer: bool
            whether to return a short answer or a long answer. Short answers are one or at most two words, very concise.
            Long answers are longer, and may be paragraphs and explanations. Defalt is True (so long answer).

        Examples
        --------
        >>> # What is the city this building is in?
        >>> def execute_command(image) -> str:
        >>>     image_patch = ImagePatch(image)
        >>>     building_patches = image_patch.find("building")
        >>>     building_patch = building_patches[0]
        >>>     building_name = building_patch.simple_query("What is the name of the building?")
        >>>     return building_patch.llm_query(f"What city is {building_name} in?", long_answer=False)

        >>> # Who invented this object?
        >>> def execute_command(image) -> str:
        >>>     image_patch = ImagePatch(image)
        >>>     object_patches = image_patch.find("object")
        >>>     object_patch = object_patches[0]
        >>>     object_name = object_patch.simple_query("What is the name of the object?")
        >>>     return object_patch.llm_query(f"Who invented {object_name}?", long_answer=False)

        >>> # Explain the history behind this object.
        >>> def execute_command(image) -> str:
        >>>     image_patch = ImagePatch(image)
        >>>     object_patches = image_patch.find("object")
        >>>     object_patch = object_patches[0]
        >>>     object_name = object_patch.simple_query("What is the name of the object?")
        >>>     return object_patch.llm_query(f"What is the history behind {object_name}?", long_answer=True)
        """
        return llm_query(question, long_answer)


def best_image_match(list_patches: List[ImagePatch], content: List[str], return_index=False) -> Union[ImagePatch, int]:
    """Returns the patch most likely to contain the content.
    Parameters
    ----------
    list_patches : List[ImagePatch]
    content : List[str]
        the object of interest
    return_index : bool
        if True, returns the index of the patch most likely to contain the object

    Returns
    -------
    int
        Patch most likely to contain the object
        
    Examples
    --------
    >>> # What is the blue foo doing?
    >>> def execute_command(image) -> str:
    >>>     image_patch = ImagePatch(image)
    >>>     foo_patches = image_patch.find("foo")
    >>>     foo_patch = best_image_match(foo_patches, ["blue"])
    >>>     return foo_patch.simple_query("What is the foo doing?")
    """
    return best_image_match(list_patches, content, return_index)


def distance(patch_a: ImagePatch, patch_b: ImagePatch) -> float:
    """
    Returns the distance between the edges of two ImagePatches. If the patches overlap, it returns a negative distance
    corresponding to the negative intersection over union.

    Parameters
    ----------
    patch_a : ImagePatch
    patch_b : ImagePatch
    
    Returns
    ----------
    float
        The distance of the two patches.

    Examples
    --------
    >>> # Return the qux that is closest to the foo
    >>> def execute_command(image):
    >>>     image_patch = ImagePatch(image)
    >>>     qux_patches = image_patch.find('qux')
    >>>     foo_patches = image_patch.find('foo')
    >>>     foo_patch = foo_patches[0]
    >>>     qux_patches.sort(key=lambda x: distance(x, foo_patch))
    >>>     return qux_patches[0]
    """
    return distance(patch_a, patch_b)


def bool_to_yesno(bool_answer: bool) -> str:
    """
    Convert a boolean value to "yes" or "no"

    Parameters
    ----------
    bool_answer : bool
    
    Returns
    ----------
    str
        "yes" or "no"

    Examples
    --------
    >>> # Is the buz green?
    >>> def execute_command(image):
    >>>     image_patch = ImagePatch(image)
    >>>     buz_patches = image_patch.find('buz')
    >>>     buz_patch = best_image_match(buz_patches, ["buz"])
    >>>     return bool_to_yesno(buz_patch.verify_property("buz", "green"))
    """
    return "yes" if bool_answer else "no"


def coerce_to_numeric(string):
    """
    This function takes a string as input and returns a float after removing any non-numeric characters.
    If the input string contains a range (e.g. "10-15"), it returns the first value in the range.
    """
    return coerce_to_numeric(string)

Write a function using Python and the ImagePatch class (above) that could be executed to provide an answer to the query. 

Consider the following guidelines:
- Use base Python (comparison, sorting) for basic logical operations, left/right/up/down, math, etc.
- Use the llm_query function to access external information and answer informational questions not concerning the image.

Query: INSERT_QUERY_HERE
\end{minted}

==> prompts/prompt_rcode.tex <==
\begin{minted}[breaklines, breaksymbolleft={}, breaksymbolright={}, fontsize=\footnotesize, escapeinside=||]{markdown}
Write some examples of a question and Python code using the API reference above that provides the answer to the question.

Consider the following guidelines:
- Must use all class, methods, fields, and functions above at least
  one time.
- Must refer to code example above.
- Must write at least three example.
\end{minted}


==> prompts/prompt_rpre.tex <==
\begin{minted}[breaklines, breaksymbolleft={}, breaksymbolright={}, fontsize=\footnotesize, escapeinside=||]{markdown}
Rewrite the API reference above.

Consider the following guidelines:
- Make the API reference shortly.
- Must include all class, methods, fields, and functions above.
- Must include some explanations to make clear the usage of each
  class, methods, fields, and functions above.
\end{minted}

==> prompts/prompt_rsp.tex <==
\begin{minted}[breaklines, breaksymbolleft={}, breaksymbolright={}, fontsize=\footnotesize, escapeinside=||]{markdown}
- Must make {type_definition[i]}
\end{minted}


==> prompts/prompt_type.tex <==
\begin{minted}[breaklines, breaksymbolleft={}, breaksymbolright={}, fontsize=\scriptsize, escapeinside=||]{markdown}
- obj: Question asking existence of object.
- cat: Question related to object identification within some category.
- attr: Question asking about the attributes or position of an object. (e.g. "What is the color of bar?", "On which of image is the foo?")
- rel: Question derived from an affirmative sentence and asking about its subject or object (e.g. “What is the foo next to the baz wearing?”, “Is the qux holding a quux?”).
- global: Question asking about the entire situation of the scene, such as weather or facility (e.g. “Is it foo?”).
\end{minted}

==> tab/tab_classification.tex <==
\begin{table}[t]
\centering
\caption{Question type classification accuracy.}
\label{tab:classification}
\begin{tabular}{l|ccc}
\toprule
\multirow{2}{*}{LLM} & \multicolumn{3}{c}{Accuracy (\%)}\\
& GQA & VQAv2 & NLVR2\\
\midrule
gpt-3.5-turbo & 58.1 \\
gpt4.0-turbo & \\
claude-3-opus &\\
\bottomrule
\end{tabular}
\end{table}



==> tab/tab_llm.tex <==

\begin{table}[t]
\setlength{\tabcolsep}{5pt}
\centering
\caption{Cross LLM evaluation (GQA dataset, gpt-3.5-turbo).}
\label{tab:llm}
\begin{tabular}{l|ccc}
\toprule
Inference/Compress & gpt-3.5-turbo & gemini-pro & claude-2.1 \\
\midrule
gpt-3.5-turbo & 43.6 \\
gemini-pro \\
claude \\
\bottomrule
\end{tabular}
\end{table}

==> tab/tab_preprompt.tex <==
\begin{table}[t]
\centering
\caption{Evaluation using different preprompts.}
\label{tab:preprompt}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l|cc|c}
\toprule
Preprompt definition & Token length & Characters & Accuracy (\%)\\
\midrule
ViperGPT preprompt & 3,434 & 15,950 & 41.3\\
w/ AdaCoder & 992 & 4,337 & 43.6\\
\midrule
VisProg preprompt & 1,212 & 5,171 & \red{WIP}\\
w/ AdaCoder & 224 & 980 & \red{WIP}\\
\bottomrule
\end{tabular}
\end{table}
% rel, 224, 990
% obj, 197, 867
% global, 211, 947
% cat, 246, 1101
% attr, 242, 993

